A Survey of the Metrics, Uses, and Subjects of Diversity-Based Techniques in Software Testing

There has been a significant amount of interest regarding the use of diversity-based testing techniques in software testing over the past two decades. Diversity-based testing (DBT) technique uses similarity metrics to leverage the dissimilarity between software artefacts - such as requirements, abstract models, program structures, or inputs - in order to address a software testing problem. DBT techniques have been used to assist in finding solutions to several different types of problems including generating test cases, prioritising them, and reducing very large test suites. This paper is a systematic survey of DBT techniques that summarises the key aspects and trends of 144 papers that report the use of 70 different similarity metrics with 24 different types of software artefacts, which have been used by researchers to tackle 11 different types of software testing problems. We further present an analysis of the recent trends in DBT techniques and review the different application domains to which the techniques have been applied, giving an overview of the tools developed by researchers to do so. Finally, the paper identifies some DBT challenges that are potential topics for future work.

==> LTS-example.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=0.45\columnwidth]{LTS.pdf}
  
    \caption{
        \label{fig:LTS-example}
        An example of a Labelled Transition System (LTS).
    }
\end{figure}

==> papers-per-artifact.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=1.\columnwidth]{publication-per-artifact.pdf}
  
    \caption{
        \label{fig:papers-per-artifact}
        The number of diversity-based papers published using different diversity artifacts.
    }
\end{figure}

==> papers-per-problem.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=1.\columnwidth]{problem-papers.pdf}
  
    \caption{
        \label{fig:papers-per-probelm}
        The number of diversity-based papers published in software testing problems.
    }
\end{figure}
